Roofline Model for UAVs: A Bottleneck Analysis Tool for Onboard Compute Characterization of Autonomous Unmanned Aerial Vehicles

We introduce an early-phase bottleneck analysis and characterization model called the F-1 for designing computing systems that target autonomous Unmanned Aerial Vehicles (UAVs). The model provides insights by exploiting the fundamental relationships between various components in the autonomous UAV, such as sensor, compute, and body dynamics. To guarantee safe operation while maximizing the performance (e.g., velocity) of the UAV, the compute, sensor, and other mechanical properties must be carefully selected or designed. The F-1 model provides visual insights that can aid a system architect in understanding the optimal compute design or selection for autonomous UAVs. The model is experimentally validated using real UAVs, and the error is between 5.1\% to 9.5\% compared to real-world flight tests. An interactive web-based tool for the F-1 model called Skyline is available for free of cost use at: ~\url{https://bit.ly/skyline-tool}

==> backup.tex <==
\begin{figure}[t]
\vspace{5pt}
        \includegraphics[width=0.95\columnwidth]{figs/annotated_drone_fig.png}
        \vspace{-10pt}
        \caption{Details of the drone build. \vspace{-20pt}}
        \label{fig:drone-setup}
\end{figure}


\begin{table}[t!]
\resizebox{0.95\textwidth}{!}{%
\LARGE
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}UAV\\ Name\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Type\\ \end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Size\\ (mm)\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ (g)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Battery\\ Capacity\\ (mAh)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Onboard\\ Compute\end{tabular}} \\ \hline
\hline
\textit{AscTec Pelican}~\cite{high-speed-drone} & mini-UAV &650 & 1652 & 6250 & Intel NUC \\ \hline
\textit{3DR Iris}~\cite{trailnet} & mini-UAV &560 & 1282 & 5100 & Nvidia Jetson TX1 \\ \hline
\textit{Parrot Bebop 1.0}~\cite{cad2rl} & mini-UAV &380 & 400 & 2700 & ARM Cortex 9+ GPU \\ \hline
\textit{Parrot Bebop 2.0}~\cite{cad2rl,dronet} & mini-UAV & 380 & 500 & 2700 & Intel Core-i7 (offload) \\ \hline
\textit{DJI Spark}~\cite{dji-spark} & micro-UAV &170 & 300 & 1480 & Intel Movidius VPU \\ \hline
\textit{BitCraze CrazyFlie}~\cite{airlearning,sourceseeking} & nano-UAVs &90 & 27 & 240 & Cortex-M4 \\ \hline
\end{tabular}%
}
%\vspace{-10pt}
\caption{Diversity of UAVs in terms of its size, weight, power, and onboard compute platforms.\vspace{-20pt}}
\label{tab:swap}
\end{table}




\begin{figure}[t]
%    \begin{subfigure}{.2\linewidth}
%        \includegraphics[width=1.5in]{figs/rebuttal/fig5-a.pdf}
%        \caption{\footnotesize F-1 roofline.}
%        \label{fig:bd-bound}
%    \end{subfigure}
    \hspace{-20pt}
    \begin{subfigure}{.2\linewidth}
        \includegraphics[width=1.0in]{figs/bounds.pdf}
        \caption{\footnotesize Different bounds.}
        \label{fig:sen-bound}
    \end{subfigure}
    \hspace{10pt}
    \begin{subfigure}{.21\linewidth}
        \includegraphics[width=1.4in]{figs/optimality.png}
        \caption{\footnotesize Optimal design.}
        \label{fig:optimal-design}
     \hspace{10pt}
    \end{subfigure}
    \begin{subfigure}{.21\linewidth}
    \includegraphics[width=1.4in]{figs/eff-a.png}
    \caption{\footnotesize Effect of a$_{max}$.}
    \label{fig:eff-a}
    \end{subfigure}
\hspace{10pt}   

%\begin{subfigure}{0.2\linewidth}
%    \includegraphics[width=1.4in]{figs/eff-d}
%    \caption{\footnotesize Effect of \textit{d}.}
%    \label{fig:eff-d}
%\end{subfigure}
        %\hspace{-13pt}
        %\begin{subfigure}{.25\linewidth}
        %\includegraphics[width=1.54in]{figs/rebuttal/fig5-d.pdf}
        %\caption{\footnotesize Effect of a$_{max}$.}
        %\label{fig:eff-a}
    %\end{subfigure}
%    \begin{subfigure}{.19\linewidth}
%        \includegraphics[width=1.31in]{figs/fig4/effect_of_d_2.pdf}
%        \caption{\footnotesize \vspace{-0.05in}Effect of d.}
%        \label{fig:eff-d}
%    \end{subfigure}
\vspace{-10pt}
     \caption{(a) Using F-1 model to understand different bounds namely compute, sensor and physics bound respectively. (b) Determining optimal design using F-1 model. (c) Effects of a$_{max}$.} %(d) Effect of range (\textit{d}).\vspace{-10pt}}
    \label{fig:f1-model}
\end{figure}
